A Girl Has A Name: Detecting Authorship Obfuscation

Authorship attribution aims to identify the author of a text based on the stylometric analysis. Authorship obfuscation, on the other hand, aims to protect against authorship attribution by modifying a text's style. In this paper, we evaluate the stealthiness of state-of-the-art authorship obfuscation methods under an adversarial threat model. An obfuscator is stealthy to the extent an adversary finds it challenging to detect whether or not a text modified by the obfuscator is obfuscated - a decision that is key to the adversary interested in authorship attribution. We show that the existing authorship obfuscation methods are not stealthy as their obfuscated texts can be identified with an average F1 score of 0.87. The reason for the lack of stealthiness is that these obfuscators degrade text smoothness, as ascertained by neural language models, in a detectable manner. Our results highlight the need to develop stealthy authorship obfuscation methods that can better protect the identity of an author seeking anonymity.

==> Sections/6_tables.tex <==
\begin{table}
\scriptsize
\begin{tabular}{|c|p{3cm}|c|c|c|}
\hline
\textbf{Dataset}                         & \multicolumn{1}{c|}{\textbf{Models}}             & \textbf{P} & \textbf{R} & \textbf{F1}   \\ \specialrule{1.5pt}{1pt}{1pt}
\multirow{5}{*}{\makecell{\amt \\[0ex]obfuscated}}& \bertlarge + ranks + VGG-19 + \rfc      & 1.00      & 0.85   & \textbf{0.92} \\ \cline{2-5} 
                                & \bertlarge + ranks + VGG-19 + \svm      & 0.98      & 0.83   & \textbf{0.90} \\ \cline{2-5}
                                & GLTR + \svm                              & 1.00      & 0.70   & 0.83 \\ \cline{2-5} 
                                & Writeprints + \svm           & 0.67      & 0.38   & 0.49 \\ \cline{2-5} 
                                & Character trigrams + \knn     & 0.64      & 0.15   & 0.24 \\ \specialrule{1.25pt}{1pt}{1pt}
\multirow{5}{*}{\makecell{\amt \\[0ex]evaded}}    & \bertlarge + probs + bins(0.010) + \nueralnetworks   & 1.00      & 0.90   & \textbf{0.95}  \\ \cline{2-5} 
                                & \bertsmall + probs + VGG-19 + \naivebayes  & 1.00      & 0.90   & \textbf{0.95} \\ \cline{2-5} 
                                & GLTR + \svm                              & 1.00      & 0.80   & 0.89 \\ \cline{2-5} 
                                & Writeprints + \svm           & 0.79      & 0.63   & 0.70 \\ \cline{2-5} 
                                & Character trigrams + \knn    & 1.00      & 0.17   & 0.29 \\ \specialrule{1.25pt}{1pt}{1pt}
\multirow{5}{*}{\makecell{\blogs \\[0ex]obfuscated}}& \bertsmall + probs + VGG-19 + \nueralnetworks                  & 0.85      & 0.71   & \textbf{0.77} \\ \cline{2-5} 
                                & \bertsmall + probs + VGG-19 + \svm             & 0.79      & 0.74   & \textbf{0.77} \\ \cline{2-5} 
                                & GLTR + \svm                                        & 0.92      & 0.40   & 0.56 \\ \cline{2-5} 
                                & Writeprints + \svm           & 0.71      & 0.41   & 0.52 \\ \cline{2-5} 
                                & Character trigrams + \knn    & 0.41      & 0.50   & 0.45 \\ \specialrule{1.25pt}{1pt}{1pt}
\multirow{5}{*}{\makecell{\blogs \\[0ex]evaded}}  & \gptlarge + ranks + VGG-19 + \naivebayes      & 0.82      & 0.83   & \textbf{0.83} \\ \cline{2-5} 
                                & \bertsmall + probs + VGG-19 + \nueralnetworks             & 0.79      & 0.81   & \textbf{0.80} \\ \cline{2-5} 
                                & GLTR + \svm                                        & 0.86      & 0.55   & 0.67 \\ \cline{2-5} 
                                & Writeprints + \svm           & 0.84      & 0.62   & 0.71 \\ \cline{2-5} 
                                & Character trigrams + \knn    & 0.86      & 0.50   & 0.63 \\ \specialrule{1.25pt}{1pt}{1pt}
\end{tabular}
\centering
	\caption{Obfuscation detection experiment results (P: precision, R: recall, F1: F1 score).}\label{main_results}
	
\end{table}

==> related_backup.tex <==
\section{Related Work}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Authorship Obfuscation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The task of authorship obfuscation aims at changing the input document, using text transformations such that the output document successfully evades attribution while preserving original semantics.
%
On the basis of the way these text-transformations are applied, current research on authorship obfuscation can be divided into two types 1) Manual/Semi-automated Methods and 2) Automated Methods.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Among manual methods, \cite{brennan2012adversarial} tries to achieve obfuscation by instructing humans to either imitate the writing style of some author or just try to hide their own writing style.
%
Among semi-automated methods, \cite{mcdonald2012use} presents a tool called Anonymouth which analyzes the input document using an authorship attribution method and then suggest text-based changes.
%
% These changes help in changing stylometric features which are giving away the identity of author.
%
Main limitation of manual and semi-automated methods is that they require human input for applying text transformations due to which these methods are not very scalable.
%
This has lead the research in authorship obfuscation towards automated methods.
%
Automated authorship obfuscation methods are the ones in which no human input is required to apply text transformations.
%
% Although automated methods targeting authorship obfuscation were introduced earlier \cite{brennan2012adversarial}, the real surge in these methods came in the last five years.
%
Existing automated methods can be further classified into rule-based and search-based.

In order to achieve obfuscation, \cite{karadzhov2017case} uses rule-based text transformations to push the style of input document towards the average style of corpus.
%
% Then they use a set of rule-based text transformations (e.g., replace ! with !!, merge or split sentences etc.) to move the stylometric feature values (e.g., punctuation to word count ratio, average number of words per sentence etc. ) of input document towards the average of corpus.
%
\cite{castro2017author} presents another rule-based approach which tries to achieves obfuscation by applying text transformations which aim to simplify the input document.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vspace{0.05in} \noindent \textbf{Model-based.}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \cite{shetty2018a4nt} makes use of Generative Adversarial Networks (GANs) for authorship obfuscation.
% %
% They used auto-encoders to generate text which are trained using three different feedbacks.
% %
% Each of these feedback respectively makes sure that the generated text evades attribution, preserves semantics and is smooth.
% %
% \cite{emmery2018style} also uses auto-encoders to generate text but they use a Gradient Reversal Layer (GRL) to make sure that the generated text does not contain any writing style signature.
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \vspace{0.05in} \noindent \textbf{Search-based.}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In search-based methods, \cite{mahmood2019girl} uses genetic algorithms (GA) along with an authorship attribution method to identify words in a document, changing which will have the maximum adverse effect on authorship attribution.
%
Sentiment preserving word embeddings are then used for word replacement.
% Words are changed by replacing them with nearest neighbors using pre-trained word embeddings.
%
\cite{bevendorff2019heuristic} tries to achieve obfuscation by increasing the stylistic distance between input document and author's existing text.
%
To achieve this, they use a heuristic based search algorithm to find the optimal set of text transformations and words to change.
%
Possible text transformation include n-gram removal, context dependent word replacement etc.

Apart from these, there are also a couple of model-based approaches \cite{shetty2018a4nt, emmery2018style} which train a deep learning model to generate obfuscated documents.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Obfuscation Detection}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\cite{juola2012detecting} uses stylometric features to perform obfuscation detection on manually obfuscated documents.
%
Their method was able to successfully detect 83\% of the obfuscated documents.
% \cite{juola2012detecting} performs obfuscation detection by applying K Nearest Neighbors (KNN) using cosine distance on the writing style of original and manually generated obfuscated documents.
%
% After applying text pre-processing steps i.e., unify case and separate consecutive punctuation characters with space, writing style is extracted using character 3-grams.
%
\cite{afroz2012detecting} also performs manual obfuscation detection using stylistic features.
%
Their approach achieves F-measure of 97\%.
%They performed experiments with three different feature sets i.e, writeprints feature set \cite{zheng2006framework}, lying-detection feature set \cite{burgoon2003detecting}\cite{hancock2007lying} and 9-feature set \cite{brennan2009practical}.
%
% Support Vector Machine (\svm) with \textit{poly} kernel using writeprints feature set performed the best, achieving an overall F-measure of 96.6\%.
%
These methods work great for manual obfuscation but as we show in our experiments, they do not perform as well against automated obfuscation methods.
%

Text spinning can also be seen as authorship obfuscation problem.
%
\cite{shahid2017accurate} uses stylometric analysis to detect whether a document was generated using text spinners or not.
%
They first extract a number of text-based features belonging to six classes i.e., n-grams, lexical, vocabulary richness, readability, syntactic and perplexity.
%
Then a \svm is applied using the radial basis function (RBF) kernel.
%
They were able to detect spun documents with F1-score of 99.94\%.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Machine Generated Text Detection}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\cite{gehrmann2019gltr} helps humans in detecting whether a given piece of text is written by a human or a particular language model called GPT-2.
%
They achieve this by extracting probability distribution of words given their context, using a pre-trained GPT-2 \cite{radford2019language} and then providing this information to humans.
%
Using this approach, authors were able to increase human detection rate from 54\% to 72\%.
% self note -- This needs work -- how it differs from our work
\cite{zellers2019defending} performs neural fake news detection by identifying if the given news article is written by a human or their fake news generation model called GROVER.
%
For an input document, they used their model GROVER to extract features from the final hidden state, which are then used to perform classification.
%
This paper showed that GROVER based detector was able to detect fake news generated by GROVER better than GPT-2 and BERT.
%
\cite{bakhtin2019real} also tries to distinguish between human and language model generated text.
%
They do this by training a separate detection model instead of relying on the output from language model.




%While prior research has shown that stylometric methods can successfully detect manually obfuscated documents (because humans tend to follow a particular writing style when trying to obfuscate a document \cite{afroz2012detecting}), it is unclear whether this pattern holds for documents obfuscated using authorship obfuscation tools \asad{because text transformations in these tools are applied by machines.
%On the other hand, it might be possible for these obfuscation tools to make some specific kind of changes, to successfully obfuscate documents, which gives them a unique writing style.}
%
% On the other hand, it is also possible that these automated obfuscators have different individual writing styles instead of one unique writing style.}
%Prior research has shown that synthetic text generated using neural language models can be successfully detected because language models usually tend to choose words with high probabilities to make sure that the generated text is coherent (or ``smooth") \cite{gehrmann2019gltr}.
%However, it is unclear whether this pattern holds for documents obfuscated using authorship obfuscation tools because synthetic text only have to be coherent whereas obfuscated text has the added constraint of evading attribution while preserving the original semantics.


%Obfuscation detection is different than generated text detection in that the generated texts only have to be smooth whereas obfuscated texts have the added constraint of evading attribution while preserving the original semantics.



%Another similar line of research is generated text detection.
% - differentiating from generated text detection
%GLTR \cite{gehrmann2019gltr} tries to perform fake text detection by finding out if the text was generated by a language model or not, using the language model itself.
%
%For text generation, 
%
%GLTR uses this information to differentiate between human and language model generated text.

%\vspace{0.05in} \noindent \textbf{Proposed Approach.} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




% Our intuition is that automated obfuscation methods, in their pursuit of evading authorship attributers, make certain changes in the text which degrade the overall smoothness of text.
% %
% This is probably because the transformations used by current obfuscation methods aren't as good as humans.
% %
% The added requirement that the obfuscated document should evade attribution also restricts the universe of transformations in some way.

==> results_old.tex <==

\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{images/LanguageModels.pdf}
  \caption{Notched box plots of F1 scores for each language model for all experiment combinations (40) across the 4 datasets.}\label{lm}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{images/LanguageModels_outputs.pdf}
  \caption{Notched box plots of F1 scores for word likelihood types for all experiment combinations (80) across the 4 datasets.}\label{lmot}
\end{figure}


\section{Results}
After averaging the F1 scores achieved by all 160 parameter combinations for each dataset, we find that 25\% achieve F1 score greater than 0.74, 50\% achieve F1 score greater than 0.70 whereas 25\% of them were able to achieve F1 score greater than 0.49.
% Across all 640 experiments (160 parameter combinations for each dataset), we find that 25\% ?? 50\% achieve an F1 score greater than 0.65
% while 75\% achieve an F1 score of 0.5 or more. has to be dataset independent.  recalculate.
%
Thus it shows that a higher percentage of our proposed architectures (160 in total) were able to perform well.

Instead of a random selection for architecture we make a strong assumption that the adversary is knowledgeable about the various choices, tests these alternatives and employs the best configuration. 
%This indicates that ...
%which shows that there are relatively less number of experiments having F1 score less than 0.5 as compared to experiments having f1 score greater than 0.5.
Thus, we present results for the best models achievable by the adversary in Table 1.

%Adversary trying to perform obfuscation detection has access to 4 language models each of which give 2 types of outputs.
%
%These outputs can be used to extract 4 different features sets which can be used with any of 5 different classifiers.
%
%So in total, adversary has access to 160 unique architectures and can pick the best one.
%
%Hence from our architectures, we show results only for the top performing ones.
%
The best architectures are chosen on the basis of F1 score.
%
For each dataset, table \ref{main_results} shows precision, recall and F1 score for our two best performing architectures and for the other methods presented in section \ref{other_methods}.


When comparing the F1 score or recall, our best performing BERT and GPT2 combination outperforms all other methods across all the four datasets.
%
But in precision, the methods using GLTR based features outperform others consistently however in each case with a penalty paid in recall.
%

Table \ref{main_results} also shows that obfuscation detection is easier in \amt dataset than in \blogs dataset.
%
This can be explained by the nature of documents in each dataset. %
\amt dataset comprises of scholarly articles which are relatively more consistent in smoothness than blogs.
%
Hence, it is easier to differentiate between original and obfucated documents on the basis of smoothness in \amt dataset than in \blogs dataset.
%
We can also see that evaded documents achieve higher F1 scores than obfuscated documents.
%
This confirms our intuition presented in \ref{obfandevaded}, that evaded documents are less smooth and therefore easier to detect than obfuscated documents.



%Hence, if it is important not to misclassify original documents as obfuscated (false positives), then choosing the model with high precision is right.
%
%On the other hand, if you need to successfully detect obfuscated documents without caring about the misclassification of original documents  i.e., less false negatives, then using the model with high recall makes more sense.

\subsection{Detector Architecture Choices Analysis}
Now we analyze the effect of different choices made within each of the three dimensions depicted in figure \ref{pipeline}.
%
More specifically, we analyze choices on the basis of highest F1 score achieved and F1 score variability.
%
We also check for significant differences between median F1 scores on the basis of notched box plots \cite{krzywinski2014points}.
%
This analysis is based on all 640 experiments described in section \ref{mfoa}.

\subsubsection{Dimension 1: Language model and output type}

%In our experiments, we tested with 4 different langauge models i.e., bert base, bert large, GPT-2 117M and GPT-2 345M.
%
Figure \ref{lm} presents notched box plots comparing distributions of F1 scores achieved by the language models across all four datasets.
%by experiments using these langauge models .
%
\bertlarge achieves the highest F1 score of 0.91 and 0.93 on \amt obfuscated and evaded datasets respectively.
%
The highest F1 score for \blogs obfuscated is achieved by \bertsmall (0.76) and for \blogs evaded by \gptlarge (0.81).
%
In terms of F1 score variability (box size) we see that for \amt datasets, BERT shows greater consistency than when using GPT-2.
%
In contrast, all models are similar in box size for \blogs datasets.
%
The only significant difference found is where \amt obfuscated, where median F1 for \bertlarge is significantly better than for \gptsmall.
%
%\vspace{0.05in} \noindent \textbf{2) Ranks versus probabilities as output:}
%We tested with two output types i.e., probabilities and ranks
%

There is no difference in maximum F1 score when using probabilities or ranks as the information output by the language models - for the evaded datasets (see Figure \ref{lmot}).
%
With obfuscated datasets using ranks is the best (0.91) for \amt whereas probabilities win for \blogs (0.76).
%experiment,  were able to achieve the highest F1 score of 0.76.
%
Box sizes show that F1 scores have a relatively smaller spread with probabilities than with ranks across all four datasets.

\subsubsection{Dimension 2: Feature type}
% We tested with two different feature representations i.e., binning and VGG-19 features.
%
%Notched box plots in figure \ref{ft} show the comparison of F1 scores between binning and image based feature representations across all four datasets.
%
From figure \ref{ft} we see that 
for \amt obfuscated, binning based features is the best (highest F1 score of 0.91) whereas for \blogs obfuscated, image based features is the best (highest F1  of 0.76).
%
There is no difference between the two for the evaded datasets.
%
Across all the four datasets, the box sizes show that experiments using image based feature representation achieve less variable F1 scores than binning based features which can be explained with the different choices of bin sizes.
%
Additionally, it can also be seen that image based features achieve significantly higher median F1 score than binning based features, across all datasets.

\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{images/Feature_type.pdf}
  \caption{Notched box plots of F1 scores for feature types for all experiment combinations (binning based: 120, image based: 40) across the 4 datasets.}\label{ft}
\end{figure}


\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{images/Classifier.pdf}
  \caption{Notched box plots of F1 scores for classifiers used for all experiment combinations (32) across the 4 datasets.}\label{c}
\end{figure}

\subsubsection{Dimension 3: Classifier}
% For classification, we used a range of different classifiers including GNB, KNN, ANN, SVM, RFC and DC(mahalanobis).
%
Figure \ref{c} shows the range of F1 scores achieved by each classifier across the four datasets.
%
For \amt obfuscated, \knn and \nueralnetworks achieve the highest F1 score of 0.91 whereas for \amt evaded, \nueralnetworks and \rfc achieve the highest F1 score (0.93).
%
For \blogs obfuscated, \svm achieves the highest F1 score of 0.76 and for \blogs evaded, \knn and \naivebayes achieve the highest F1 score of 0.81.
%
As for the variability in F1 scores, \knn and \nueralnetworks consistently achieve relatively stable F1 scores than the other classification methods.
%
In \amt dataset, \knn and \nueralnetworks both achieve significantly higher median F1 score than \svm and \rfc.
%
Additionally, in \amt evaded, \knn also achieves significantly higher median F1 score than \naivebayes.
%
In \blogs dataset, \knn and \ann achieve significantly higher median F1 score than \svm, \rfc and \naivebayes.

\vspace{0.05in} \noindent \textbf{Optimal Architecture:}
We aim to choose the combination of choice variables which gives good results across all four datasets.
%
To this end we choose variables which have two qualities.
%
1) Their maximum F1 score is equal or closer to the overall maximum F1 score achieved.
%
2) They have a relatively tighter range of F1 scores i.e, smaller box sizes.
%
Hence we pick the following combination: \bertsmall + probabilities + VGG-19 + \nueralnetworks.
%
This combination was able to achieve the F1 scores of 0.84, 0.91, 0.74 and 0.75 for \amt obfucated, \amt evaded, \blogs obfuscated and \blogs evaded respectively.
% 
These F1 scores beat the second best model i.e., model using GLTR across all the four datasets.


\subsection{Intuition Analysis}
Earlier in section \ref{propapproach} we explained that our intuition behind obfuscation detection is that the text generated by obfuscaters and humans differ in terms of fluency.
%
We defined fluency as the number of high likelihood words used which are extracted by a pre-trained language model.
%
Figure \ref{intuit} verifies this intuition.
%
For this plot, we first extract the occurrence probabilities of words using \bertsmall and sort them for all the documents in \amt obfuscated dataset.
%
Then we average these sorted probabilities for different obfuscator generated and original documents and plot them.
%
The steeper the fall, the greater the average number of low probability words in documents and hence lower the smoothness of text.
%
This plot shows that original documents are more smooth on average whereas \dspan generates the least smooth documents.

\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{images/average_VGG.pdf}
  \caption{Comparison between different obfuscators and original documents on the basis of average sorted probabilities extracted by \bertsmall for \amt obfuscated dataset.}\label{intuit}
\end{figure}
